Robust Markov Decision Processes without Model Estimation

Robust Markov Decision Processes (MDPs) are receiving much attention in learning a robust policy which is less sensitive to environment changes. There are an increasing number of works analyzing sample-efficiency of robust MDPs. However, there are two major barriers to applying robust MDPs in practice. First, most works study robust MDPs in a model-based regime, where the transition probability needs to be estimated and requires a large amount of memories $\mathcal{O}(|\mathcal{S}|^2|\mathcal{A}|)$. Second, prior work typically assumes a strong oracle to obtain the optimal solution as an intermediate step to solve robust MDPs. However, in practice, such an oracle does not exist usually. To remove the oracle, we transform the original robust MDPs into an alternative form, which allows us to use stochastic gradient methods to solve the robust MDPs. Moreover, we prove the alternative form still plays a similar role as the original form. With this new formulation, we devise a sample-efficient algorithm to solve the robust MDPs in a model-free regime, which does not require an oracle and trades off a lower storage requirement $\mathcal{O}(|\mathcal{S}||\mathcal{A}|)$ with being able to generate samples from a generative model or Markovian chain. Finally, we validate our theoretical findings via numerical experiments, showing the efficiency with the alternative form of robust MDPs.

==> tex/bandit_old.tex <==
Let's consider a bandit case with parameters $\langle\XM, R, P\rangle$. We assume the reward function $R:\XM\to\RB_{+}$ is deterministic. Our fundamental interest is to evaluate the following objective:
\begin{align*}
    L(P,\rho):=\inf_{D_f(Q\|P))\le\rho} \EB_Q R(X).
\end{align*}
We can also write the dual form of $L(P,\rho)$ by:
\begin{align*}
    D(P,\rho):=\sup_{\lambda\ge0,\eta\in\RB}-\lambda \EB_P f^*\left(\frac{\eta-R(X)}{\lambda}\right)-\lambda\rho+\eta:=\sup_{\lambda\ge0,\eta\in\RB}J(\lambda,\eta).
\end{align*}
Supposing we only access an online data stream $\{X_t\}_{t=1}^T$, we can apply Stochastic Gradient Ascent (SGA) algorithm to approximate $D(P,\rho)$:
\begin{align*}
    \lambda_{t+1}&=\left[\lambda_t+\alpha\cdot\frac{\partial J(\lambda_t,\eta_t; X_t)}{\partial\lambda}\right]_{+},\\
    \eta_{t+1}&=\eta_t+\beta\cdot\frac{\partial J(\lambda_t,\eta_t; X_t)}{\partial\eta},
\end{align*}
where $\alpha$ and $\beta$ are learning rates and can be time-dependent, and $J(\lambda_t,\eta_t;X_t):=-\lambda_t f^*\left(\frac{\eta_t-R(X_t)}{\lambda_t}\right)-\lambda_t\rho+\eta_t$, which satisfies $\EB [J(\lambda_t,\eta_t; X_t)|\FM_{t-1}]=J(\lambda_t,\eta_t)$ and $\FM_{t-1}=\sigma(\{(\lambda_0,\eta_0),...,(\lambda_t,\eta_t)\})$. Noting that the dual problem must be concave w.r.t. its dual variables \citep{boyd2004convex}, the convergence can be guaranteed.
We also make regular assumptions for $f$:
\begin{asmp}
    \label{asmp: str-convex}
    $f$ is $\sigma$-strongly convex.
\end{asmp}
\begin{asmp}
    \label{asmp: smooth}
    $f$ is $L$-smooth.
\end{asmp}
Following results of \cite{zhou2018fenchel}, we have following properties for the conjugate function $f^*$:
\begin{prop}
    If $f$ satisfies Assmuption~\ref{asmp: str-convex}, then $f^*$ is $1/\sigma$-smooth. 
\end{prop}
\begin{prop}
    If $f$ satisfies Assumption~\ref{asmp: smooth}, then $f^*$ is $1/L$-strongly convex.
\end{prop}

\begin{lem}
    The objective function $J(\lambda,\eta)$ is concave.
\end{lem}

\begin{thm}[Convergence guarantee (to do)]
    The SGA algorithm will converge to optimal point within $\OM(?)$ steps.
\end{thm}

==> tex/improve.tex <==
\begin{asmp}
    \label{asmp: monotone}
    $\nabla_{\eta} J(\eta; V)$ is $\kappa$-strongly monotone at $\eta^*_V\in\argmax_{\eta}J(\eta;V)$:
    \begin{align*}
        \nabla J(\eta; V)\cdot(\eta-\eta_{V}^*)\le-\kappa\cdot(\eta-\eta_V^*)^2
    \end{align*}
\end{asmp}
Taking $f(t)=(t-1)^2$ as an example, we have:
\begin{align*}
    J(\eta; V)&=-\lambda \EB_{s'\sim P}f^{*}\left(\frac{\eta-V(s')}{\lambda}\right)+\eta\notag\\
    &=-\frac{\EB_{s'\sim P}\left(\eta+2\lambda-V(s')\right)_{+}^2}{4\lambda}+\eta.
\end{align*}
Thus, the gradient of $J(\eta;V)$ is:
\begin{align*}
    \nabla J(\eta;V)=-\frac{\EB_{s'\sim P}\left(\eta+2\lambda-V(s')\right)_{+}}{2\lambda}+1.
\end{align*}
We observe that $\eta_V^*$ must satisfies $\eta_V^*\ge \min_{s'}V(s')-2\lambda$ or $\nabla J(\eta;V)=1$. Thus, the subgradient of $\nabla J(\eta;V)$ at $\eta_V^*$ satisfies:
\begin{align*}
    \nabla^2 J(\eta_V^*;V)\le -\frac{P(s_{\min})}{2\lambda},
\end{align*}
where $s_{\min}=\argmin_{s'} V(s')$. Then, we have Assumption~\ref{asmp: monotone} holding for $f(t)=(t-1)^2$.

\begin{algorithm}[htbp!]
    \caption{Model-free approach to robust MDPs (Improved) }
    \label{alg: improve}
    \begin{algorithmic}
        \STATE{\bfseries Input:} $Q_0(s,a)=1/(1-\gamma)$ for all $(s,a)\in\SM\times\AM$.
        \FOR{iteration $t=0$ {\bfseries to} $T-1$}
            \FOR{each $(s,a)\in\SM\times\AM$}
                \STATE Recieve reward $r(s,a)$ and next state $s'(s,a)\sim P^*(\cdot|s,a)$;
                \STATE $\eta_{t+1}(s,a)\leftarrow\Pi_{\Theta}\left(\eta_t(s,a)+\alpha_{t}\frac{\partial \widehat{J}^{(s,a)}(\eta_t(s,a); V_{t})}{\partial\eta}\right)$;
                \STATE $Q_{t+1}(s,a)=(1-\beta_{t})Q_t(s,a)+\beta_{t}(r(s,a)+\gamma \widehat{J}^{(s,a)}(\eta_t(s,a); V_t))$;
            \ENDFOR
            \STATE $V_{t+1}=\max_a Q_{t+1}(\cdot,a)$;
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

We define a filteration sequence $(\FM_{t})_{t=0}^{T}$:
\begin{align*}
    \FM_{t+1}=\sigma\left(\FM_t\cup\sigma(\{r_t(s,a), s_t'(s,a)\})\right).
\end{align*}
and $\FM_0=\sigma(\{\emptyset\})$.

\begin{asmp}
    \label{asmp: eta_lip_v}
    For any $V_1,V_2\in\VM$, there exists $L_V>0$, such that:
    \begin{align*}
        \left|\eta^*_{V_1}(s,a)-\eta^*_{V_2}(s,a)\right|\le L_V\left\|V_1-V_2\right\|.
    \end{align*}
\end{asmp}

\begin{lem}
    \label{lem: eta_error_improve}
    Denote $\delta_t(s,a)=\eta_t(s,a)-\eta_{V_t}^*(s,a)$, the following inequality holds:
    \begin{align}
        \delta_{t+1}^2(s,a)\le(1-\kappa\alpha_t)\delta_t^2(s,a)+2\alpha_t\delta_t(s,a)g_t(s,a)+2\alpha_t^2C_g^2+4\left(\frac{1}{\kappa\alpha_t}+2\right)\beta_t^2L_V^2C_M^2,
    \end{align}
    where $g_t(s,a):=\frac{\partial \widehat{J}^{(s,a)}(\eta_{t}(s,a);V_{t})}{\partial \eta}-\frac{\partial J^{(s,a)}(\eta_{t}(s,a);V_{t})}{\partial \eta}$. Moreover, denote $M_{t+1}(s,a):=(1-\kappa\alpha_t)M_t(s,a)+2\alpha_t\delta_t(s,a)g_t(s,a)$, by induction, we have:
    \begin{align*}
        \delta_{t}^2(s,a)\le\delta_0^2(s,a)\prod_{i=0}^{t-1}(1-\kappa\alpha_i)+\sum_{i=0}^{t-1}\left(2\alpha_i^2C_g^2+4\left(\frac{1}{\kappa\alpha_i}+2\right)\beta_i^2L_V^2C_M^2\right)\prod_{j=i+1}^{t-1}(1-\kappa\alpha_j)+M_t(s,a).
    \end{align*}
\end{lem}

\begin{lem}
    \label{lem: q_decomp_error}
    The following inequalities hold:
    \begin{align*}
        \Delta_{t+1}(s,a)\le&(1-\beta_t)\Delta_t(s,a)+\beta_t \left(\varepsilon_{r,t}(s,a)+\gamma \varepsilon_{J,t}(s,a)+\gamma\left\|\Delta_t\right\|_{\infty}\right)\notag\\
        \Delta_{t+1}(s,a)\ge&(1-\beta_t)\Delta_t(s,a)+\beta_t \Bigg(\varepsilon_{r,t}(s,a)+\gamma \varepsilon_{J,t}(s,a)-\frac{\gamma\left\|\eta_{t}-\eta_{V_t}^*\right\|_{\infty}^2}{2\sigma\lambda}-\gamma\left\|\Delta_t\right\|_{\infty}\Bigg).
    \end{align*}
    Moreover, by induction, we have:
    \begin{align*}
        \left\|\Delta_T\right\|_{\infty}=&\left\|\Delta_0\right\|_{\infty}\prod_{t=0}^{T-1}\left(1-(1-\gamma)\beta_t\right)+\sum_{t=0}^{T-1}\gamma\beta_t\left\|N_t\right\|_{\infty}\cdot\prod_{i=t+1}^{T-1}(1-(1-\gamma)\beta_i)\notag\\
        &+\frac{1}{2\sigma\lambda}\sum_{t=0}^{T-1}\gamma\beta_t\left\|\eta_t-\eta_{V_t}^*\right\|^2_{\infty}\cdot\prod_{i=t+1}^{T-1}(1-(1-\gamma)\beta_i)+\left\|N_T\right\|_{\infty},
    \end{align*}
    where $N_{t+1}(s,a)=(1-\beta_t)N_t(s,a)+\beta_t(\varepsilon_{r,t}+\gamma \varepsilon_{J,t})$.
\end{lem}


\begin{lem}
    \label{lem: M_concen}
    If $(1-\kappa\alpha_t)\alpha_{t-1}\le\alpha_t$, the following inequalities hold:
    \begin{align*}
        \EB\left\|M_t\right\|_{\infty}\le2\sqrt{32\kappa^{-1}\alpha_{t-1}\diam^2(\Theta)C_g^2\log(2|\SM||\AM|)}.
    \end{align*}
\end{lem}

\begin{lem}
    \label{lem: eta_rate}
    If we set $\alpha_t=\frac{1}{\kappa(t+1)^{\frac{2}{3}}}$ and $\beta_t=\frac{1}{(1-\gamma)(t+1)}$, the following inequality holds:
    \begin{align*}
        \EB\left\|\delta_t\right\|^2_{\infty}\le\frac{6C_g^2}{\kappa^2(1-\alpha)t^{\frac{1}{3}}}+\frac{12L_V^2C_M^2}{(1-\gamma)^{\frac{1}{3}}t^{\frac{1}{3}}}+\frac{32L_V^2C_M^2}{(1-\gamma)^2t^{\frac{2}{3}}}+\frac{8\sqrt{2\log(2|\SM||\AM|)}\diam(\Theta)C_g}{\sqrt{\kappa}t^{\frac{1}{3}}}.
    \end{align*}
\end{lem}

\begin{thm}
    \label{thm: q_rate}
    If we set $\alpha_t=\frac{1}{\kappa(t+1)^{\frac{2}{3}}}$ and $\beta_t=\frac{1}{(1-\gamma)(t+1)}$, the following inequality holds:
    \begin{align*}
        \EB\left\|\Delta_t\right\|_{\infty}\le\OM\left(\frac{\gamma}{2\sigma\lambda(1-\gamma)T^{\frac{1}{3}}}\left(\frac{9C_g^2 }{\kappa^2}+\frac{18L_V^2C_M^2 }{(1-\gamma)^{\frac{1}{3}}}+\frac{12\sqrt{2\log(2|\SM||\AM|)}\diam(\Theta)C_g }{\sqrt{\kappa}}\right)\right)
    \end{align*}
\end{thm}

==> tex/notation.tex <==
For any set $\XM$, we denote the set of  probability distributions on $\XM$ as $\Delta(\XM)$.
